MovieChat: From Dense Token to Sparse Memory for Long Video Understanding

Recently, integrating video foundation models and large language models to build a video understanding system can overcome the limitations of specific pre-defined vision tasks. Yet, existing systems can only handle videos with very few frames. For long videos, the computation complexity, memory cost, and long-term temporal connection impose additional challenges. Taking advantage of the Atkinson-Shiffrin memory model, with tokens in Transformers being employed as the carriers of memory in combination with our specially designed memory mechanism, we propose the MovieChat to overcome these challenges. MovieChat achieves state-of-the-art performance in long video understanding, along with the released MovieChat-1K benchmark with 1K long video and 14K manual annotations for validation of the effectiveness of our method.

==> fig/category.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/_category.pdf}
    \caption{\textbf{Category.}}
    \label{fig:category}
\end{figure}

==> fig/certi.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.88\linewidth]{fig/_certi.pdf}
    \vspace{-12pt}
    \captionsetup{font={scriptsize}}
    \caption{Certificate length across video datasets.}
    \label{fig:certi}
\end{figure}


% \begin{figure}[ht]
%     \begin{minipage}{0.5\linewidth}
%         \centering        \includegraphics[width=\linewidth]{fig/_certi.pdf}
%         \vspace{-22pt}
%         \caption{ }
%         \label{fig:certi}
%     \end{minipage}%
%     \begin{minipage}{0.5\linewidth}
%         \centering        \includegraphics[width=\linewidth]{fig/_reb_abl.pdf}
%         \vspace{-22pt}
%         \caption{ }
%         \label{fig:reb_abl}
%     \end{minipage}
% \end{figure}



==> fig/length.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/_length.pdf}
    \caption{\textbf{Average clip length.}}
    \label{fig:length}
\end{figure}

==> fig/questiontype.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/_questiontype.pdf}
    \caption{\textbf{Question type.}}
    \label{fig:questiontype}
\end{figure}

==> fig/rebuttal_abl.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{fig/_reb_abl.pdf}
    \caption{Replotting of Figure 5.}
    \label{fig:reb_abl}
\end{figure}

==> tab/class.tex <==
\begin{table}[h]
\centering
\tiny 
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{0.4}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} c c c @{}}
\toprule
 \\[-2ex]
% \hspace{1cm} \tiny \textbf{Model}\hspace{1cm} & \tiny \textbf{Text Encoder} & \tiny \hspace{1cm} \textbf{VC Acc} \hspace{1cm} \\
\tiny \textbf{Model} & \tiny \textbf{Text Decoder} & \tiny \textbf{VC Acc} \\
 \\[-2ex]
\midrule
 \\[-2ex]
\multicolumn{2}{c}{\tiny Choosing the correct answer uniformly at random} & \tiny 14.3\% \\
 \\[-2ex]
\midrule
 \\[-2ex]
\tiny GIT & \tiny non-LLM based &  \tiny 22.6\% \\
\tiny mPLUG-2 & \tiny non-LLM based & \tiny 25.3\%  \\
\tiny Video Chat & \tiny LLM based & \tiny \underline{35.6\%} \\
 \\[-2ex]
\midrule
 \\[-2ex]
\textbf{\tiny MovieChat}& \tiny LLM based & \tiny \textbf{36.4\%}  \\
 \\[-1.5ex]
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\captionsetup{font={scriptsize}}
\caption{Classification evaluation on MovieChat-1K. }
\label{tab:class}
\end{table}

% sci fic -> Science fiction film, detective film, Adventure Film
% cartoon -> Animation Film
% thriller -> Crime Film, action film
% drama -> epic film
% 去除movie， television后人工筛选

==> tab/ego.tex <==
\begin{table}[h]
\centering
\tiny
\setlength{\tabcolsep}{8pt}
\setcellgapes{0.1pt} 
\makegapedcells
\renewcommand{\arraystretch}{0.5}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} c c c @{}}
\toprule
 \\[-2ex]
% \hspace{1cm}\tiny \textbf{Model}\hspace{0.2cm}
%  & \hspace{2cm}\tiny \textbf{Text Encoder} \hspace{2cm} & \tiny \textbf{QA Acc} \hspace{3cm}\\
\tiny \textbf{Model}
 & \tiny \textbf{Text Decoder}  & \tiny \textbf{QA Acc}\\
 \\[-2ex]
\midrule
\\[-2ex]
\multicolumn{2}{c}{\tiny Choosing the correct answer uniformly at random} & \tiny  20.0\% \\
 \\[-2ex]
\midrule
 \\[-2ex]
% FrozenBiLM & non-LLM based & 26.9\% \\
% VIOLET  & non-LLM based & 19.9\% \\
% mPLUG-Owl & LLM based & 31.1\% \\
\tiny InternVideo& \tiny non-LLM based & \tiny 32.1\% \\
\tiny Video Chat & \tiny LLM based & \tiny 47.5\% \\
\tiny \textbf{MovieChat}  & \tiny LLM based & \tiny \underline{53.5\%} \\
 \\[-2ex]
\midrule
 \\[-2.5ex]
\multicolumn{2}{c}{\tiny Human Performance} & \tiny \textbf{76.2\%} \\
 \\[-2ex]
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\captionsetup{font={scriptsize}}
\caption{Zero-shot QA Evaluation on EgoSchema.}
\label{tab:ego}
\end{table}

==> tab/mplug-acc.tex <==
\begin{table}[h]
\centering
\scriptsize
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{0.7}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} c | c | c c c c @{}}
\toprule
% \multirow{}{}{\textbf{Method}} & \multirow{}{}{\textbf{\# Frames}} & \multicolumn{2}{c}{\textbf{Global Mode}} & \multicolumn{2}{c}{\textbf{Breakpoint Mode}} \\
% \cline{3-6}
%  & & \textbf{Accuracy} & \textbf{Score} & \textbf{Accuracy} & \textbf{Score} \\
\textbf{Method} & \textbf{Frames} & \textbf{Global Acc} & \textbf{Global Score} & \textbf{Breakpoint Acc} & \textbf{Breakpoint Score} \\
\midrule
\scriptsize GIT & 6 & 28.8 & 1.83 & 29.2 & 1.98 \\
\scriptsize mPLUG-2 & \scriptsize 8 & \scriptsize 31.7 & \scriptsize 2.13 & \scriptsize 30.8 & \scriptsize 1.83 \\
\scriptsize Video Chat& 32 & \underline{51.7} & \underline{2.67} & \underline{39.1} & \underline{2.04} \\
\midrule
\textbf{MovieChat~\textit{(ours)}} & 2048 & \textbf{62.3} & \textbf{3.23} & \textbf{48.3} & \textbf{2.57}\\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\captionsetup{font={scriptsize}}
\caption{Long video QA evaluation on MovieChat-1K test set.}
\label{tab:mplug-acc}
\end{table}

==> tab/mplug-short.tex <==
\begin{table}[h]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.7}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} c | c | c c @{}}
\toprule

\textbf{Method} & \textbf{Text Decoder} & \hspace{0.3cm}\textbf{MSVD-QA}\hspace{0.3cm} & \hspace{0.3cm}\textbf{MSRVTT-QA}\hspace{0.3cm} \\
\midrule

VideoCoCa & non-LLM based & 56.9 & 46.0 \\

GIT & non-LLM based & 56.8 & 43.2 \\

 mPLUG-2 &  non-LLM based &  58.1 &  48.0 \\
 
 % \rowcolor{purple!5}
 Video-ChatGPT &  LLM based &  \underline{64.9} &  \underline{49.3}\\ 
\midrule
\textbf{ MovieChat~\textit{(Ours)}} &  LLM based &  \textbf{75.2} & \textbf{52.7}\\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\captionsetup{font={scriptsize}}
\caption{Evaluation for short video question answering.}
\label{tab:mplug-short}
\end{table}

==> tab/mplug_5.tex <==
\begin{table}[h]
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{0.61}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} c | c c c c c c @{}}
\toprule
 \\[-2ex]
\hspace{0.5cm}\scriptsize \textbf{Method} \hspace{0.5cm} & \hspace{0.1cm} \scriptsize \textbf{CI} \hspace{0.1cm} & \hspace{0.1cm} \scriptsize \textbf{DO}\hspace{0.1cm} & \hspace{0.1cm} \scriptsize \textbf{CU} \hspace{0.1cm} & \hspace{0.1cm} \scriptsize \textbf{TU} \hspace{0.1cm} & \hspace{0.1cm} \scriptsize \textbf{CO} \hspace{0.5cm}\\
 \\[-2ex]
\midrule
 \\[-2ex]
\scriptsize GIT & \scriptsize 1.65  & \scriptsize 1.74  & \scriptsize 2.00  & \scriptsize 1.88  & \scriptsize 2.16 \\
\scriptsize mPLUG-2 & \scriptsize 1.82 & \scriptsize 1.93 & \scriptsize 2.24 & \scriptsize 1.92 & \scriptsize 2.35\\
\scriptsize Video Chat & \scriptsize \underline{3.04} & \scriptsize \underline{2.75} & \scriptsize \underline{3.09} & \scriptsize \underline{3.00}& \scriptsize  \underline{3.21}\\
 \\[-1.7ex]
\midrule
 \\[-1.8ex]
\hspace{0.3cm} \textbf{\scriptsize MovieChat~\textit{(Ours)}} \hspace{0.1cm}& \scriptsize \textbf{3.11}& \scriptsize \textbf{2.93} & \scriptsize \textbf{3.24}& \scriptsize \textbf{3.17}& \scriptsize \textbf{3.25} \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\captionsetup{font={scriptsize}}
\caption{Long video QA results on MovieChat-1K in global mode.}
\label{tab:mplug-5}
\end{table}

==> tab/question_type.tex <==
\begin{table}[h]
\centering
\tiny
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{0.5}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} c c | c c | c c @{}}
\toprule
 \\[-2ex]
\tiny \textbf{Type} & \tiny \textbf{Rate} & \tiny \textbf{Frame Type}& \tiny \textbf{Text Rate} & \tiny \textbf{Type} & \tiny \textbf{Text Rate}\\
 \\[-2ex]
\midrule
 \\[-2ex]
    Location & 21.2\% & Scene & 11.2\% & Existence & 5.0\% \\

    Time & 17.2\% & Object & 10.7\% & Weather & 3.6\% \\

    Number & 14.6\% & Action & 7.8\% & Others & 1.5\% \\
\\[-2ex]
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\captionsetup{font={scriptsize}}
\caption{Semantic Categorization of MovieChat-1K Questions}
\label{tab:q_type}
\end{table}

==> tex/0_abs.tex <==
\begin{abstract}
Recently, integrating video foundation models and large language models to build a video understanding system can overcome the limitations of specific pre-defined vision tasks. Yet, existing systems can only handle videos with very few frames. For long videos, the computation complexity, memory cost, and long-term temporal connection impose additional challenges. Taking advantage of the Atkinson-Shiffrin memory model,  with tokens in Transformers being employed as the carriers of memory in combination with our specially designed memory mechanism,  we propose the MovieChat to overcome these challenges. MovieChat achieves state-of-the-art performance in long video understanding, along with the released MovieChat-1K benchmark with 1K long video and 14K manual annotations for validation of the effectiveness of our method.
\end{abstract}

==> tex/1_intro.tex <==
\section{Introduction}

Recent advances in Large Language Models (LLMs)~\cite{gpt4,brown2020language,touvron2023llama,chiang2023vicuna,taori2023stanford} acheive great success in Natural Language Processing (NLP) . It is a natural progression to introduce multi-modality~\cite{chai2022deep} into LLMs and turn it into Multi-modal Large Language Models (MLLMs), which is able to conduct multimodal rationalization and understanding. MLLMs have shown incredible emergent capabilities in various multimodal tasks such as perception (\eg, existence, count, position, OCR)~\cite{wang2023visionllm, maaz2023video, alayrac2022flamingo,zhu2023minigpt,li2023otter,li2023blip}, commonsense reasoning~\cite{gao2023llama,zhu2023minigpt,li2023otter,li2022blip,li2023blip,gong2023multimodal,su2023pandagpt, maaz2023video}, and code reasoning~\cite{fu2023mme,lyu2023macaw,ye2023mplug,dai2023instructblip,liu2023visual,gao2023llama}, resulting in a potential path to Artificial General Intelligence (AGI). Compared to LLMs and other task-specific models, MLLMs  provide a more human-like interpretation of the scenarios, a user-friendly interface for interaction, and a broader range of capabilities.

\input{fig/intro}

Existing vision-centric MLLMs follow the paradigm that utilizing pre-trained LLMs and visual encoder with additional learnable modules (Q-former~\cite{dai2023instructblip,li2022blip,li2023blip,zhang2023video} or simple projection layer~\cite{driess2023palm,maaz2023video,liu2023visual,su2023pandagpt}). In video field, some previous works~\cite{zhang2023video,maaz2023video} follow this paradigm to build video MLLMs, while works in the other paradigm~\cite{wang2023chatvideo,li2023videochat} combine existing visual perception tools (\eg, tracking and classification) and LLMs through Application Programming Interface (API) to build a system without training. Yet, previously, there is no exploration of a model or system based on long videos (over one minute), and there is also a lack of a standardized benchmark to evaluate the capabilities of these systems.

In this paper, we present MovieChat, a novel framework that integrates vision models and LLMs to conduct long video understanding tasks. We claim that the computation complexity, memory cost, and long-term temporal connection are the main challenges for long video understanding. Atkinson-Shiffrin memory model~\cite{atkinson1968chapter} proposes that short-term memory functions as a buffer of long-term memory, serving as a processor for the encoding of information into long-term memory. Inspired by this, we propose a memory mechanism to deal with long video understanding tasks, which includes a rapidly updated short-term memory and a compact thus sustained long-term memory. We use a sliding window approach to extract video features and represent them in token form, which are then sequentially fed into the short-term memory frame by frame. The short-term memory has a fixed length, and when it reaches its set limit, the earliest tokens are popped and consolidated into the long-term memory. After passing through a projection layer, the video representation is inputted into a large language model for interaction with the user. As shown in Fig.~\ref{fig:intro}, our proposed MovieChat mechanism outperforms other existing methods in terms of Video Random Access Memory (VRAM) cost. We also release a new benchmark, MovieChat-1K, with 1K long videos and 13K manual question-answering pairs for validation of the effectiveness of our proposed MovieChat. 

The contributions of this work are summarized as:

\vspace{-5pt}

\begin{itemize}
    \vspace{-5pt}
    \item We present MovieChat, a novel framework that integrates vision models and LLMs, which is the first to support long video ($\textgreater 10$K frames) understanding tasks.
    \vspace{-6pt}
    \item We propose an effective memory management mechanism to reduce the computation complexity and memory cost, while enhancing the long-term connection.
    \vspace{-6pt}
    \item We release the first long video understanding benchmark, MovieChat-1K, with manual annotations and conduct extensive quantitative evaluation and case studies to evaluate the comparable performance of both understanding capability and inference cost.
\end{itemize}

==> tex/2_survey.tex <==
\vspace{-15pt}

\section{Related Works}

% \subsection{Video Foundation Models}
% Video foundation models have various applications on downstream tasks (\eg, video question answering~\cite{lei2018tvqa,lei2020tvqa+}, video captioning~\cite{iashin2020multi,yang2023vid2seq}, and human action recognition~\cite{poppe2010survey,kong2022human,qi2022weakly}). The common paradigm in the field of video foundation models is now characterized by the combination of extensive large-scale video-language pre-training, followed by fine-tuning on specific downstream tasks~\cite{miech2020end,li2020learning,xu2021videoclip,li2022uniformerv2,li2023unmasked,sun2019videobert,zhu2020actbert,wang2022internvideo}. Such paradigm depends on end-to-end video-language joint training with pretext pre-training tasks such as masked language modeling~\cite{li2023lavender}, masked video modeling~\cite{tongvideomae,wang2023videomae}, video-language masked modeling~\cite{fu2021violet}, video-text matching~\cite{wang2023all}, and video-text contrastive learning~\cite{xu2021videoclip}. These prior arts yield impressive performance in multimodal video tasks. Yet, they can only train with limited video-language pairs or videos without detailed annotations, which leads to difficulties in language-related tasks. With connecting to LLMs, video foundation models serve as visual encoder and achieve state-of-the-art performance in various tasks and become user-friendly.

% ~\cite{yin2023survey,fu2023mme,alayrac2022flamingo,zhu2023minigpt,li2023otter,li2022blip,li2023blip,gong2023multimodal,lyu2023macaw,ye2023mplug,dai2023instructblip,wang2023visionllm,liu2023visual,maaz2023video,su2023pandagpt,gao2023llama}

\subsection{Multi-modal Large Language Models}
LLMs~\cite{gpt4,brown2020language,touvron2023llama,touvron2023llama2,chiang2023vicuna,taori2023stanford} have achieved great success in natural language processing (NLP) tasks recently. Many works try to build MLLMs~\cite{alayrac2022flamingo,zhu2023minigpt,li2023otter,li2023blip,gong2023multimodal,ye2023mplug,dai2023instructblip,wang2023visionllm,maaz2023video,gao2023llama} by combining models of other modalities.
Flamingo~\cite{alayrac2022flamingo} bridges powerful pre-trained vision-only and language-only models and achieves state-of-the-art performance with few-shot learning.
BLIP-2~\cite{li2023blip} proposes a generic and efficient pre-training strategy that bootstraps vision-language pre-training from an off-the-shelf frozen pre-trained image encoders and a frozen large language model.
MiniGPT-4~\cite{zhu2023minigpt} also aligns a frozen visual encoder with a frozen LLM, Vicuna~\cite{chiang2023vicuna}, using just one projection layer to realize the system.
Otter~\cite{li2023otter} showcases improved instruction-following ability and in-context learning.
In video field, ChatVideo~\cite{wang2023chatvideo} treats tracklets as the basic video unit and allows users' interacting with the LLMs.
VideoChat~\cite{li2023videochat} integrates video foundation models and LLMs via a learnable neural interface, excelling in spatiotemporal reasoning, event localization, and causal relationship inference. 
Video-LLaMA~\cite{zhang2023video} further leverages pre-trained models ImageBind~\cite{girdhar2023imagebind} and LLaMA~\cite{touvron2023llama}, bootstraping cross-modal training in videos following BLIP-2.
Yet, these methods fail to handle long video understanding because of high computation complexity, large memory cost, and weak long-term temporal connection. Therefore, our main effort is to introduce an effective memory mechanism to overcome these challenges.

% VideoChat Longvideo~\cite{videochatlong} further incorporates LangChain~\cite{langchain} into VideoChat to handle videos exceeding one minute in length.
% \cite{wu2021towards} proposes an object-centric benchmark to cover wide but coarse tasks of long-form videos, including content understanding, user engagement prediction, and movie metadata prediction.

\vspace{-5pt}

\subsection{Long Video Understanding}
\vspace{-3pt}

Understanding long videos is a challenging task in computer vision. Prior arts use 3D CNN for long-term feature bank~\cite{wu2019long}, object/human-centric motion~\cite{wu2021towards,rohrbach2017generating}, or other forms~\cite{wu2022memvit,sener2020temporal} as video representations. MIST~\cite{gao2023mist} decomposes dense self-attention into a cascade segment and
region selection module to increase the computation efficiency for understanding minutes of long videos. Building long-form video understanding datasets is challenging and rarely explored.  \cite{shou2021generic} captures large scale data from Kinetics-400~\cite{carreira2017quo}, but only for generic event boundary detection tasks. \cite{soldan2022mad} creates a language grounding benchmark from audio descriptions of movies, but it lacks long-term understanding evaluation. \cite{tapaswi2016movieqa} successfully builds a benchmark contains multiple sources of information (\eg, video clips, plots, and DVS) for question-answering tasks in the movie field. There are also several datasets of video-caption/description pairs among various domains, such as cooking (\eg, MPII Cooking~\cite{rohrbach2012database,rohrbach2012script,rohrbach2016recognizing} and TACoS~\cite{regneri2013grounding,rohrbach2014coherent}), instruction (\eg, HowTo100M~\cite{miech2019howto100m} and HiREST~\cite{zala2023hierarchical}), Ego~\cite{mangalam2023egoschema}, and movie (\eg, MovieQA~\cite{tapaswi2016movieqa} and MovieNet~\cite{huang2020movienet}) from different sources such as YouTube~\cite{chen2011collecting,zeng2016title,miech2019howto100m}, Twitter~\cite{awad2017trecvid,awad2018trecvid,awad2020trecvid,awad2021trecvid}, and Internet~\cite{bain2021frozen}. 
Yet, those datasets lack diverse and fine-grained dense captioning for long videos.

\input{fig/overview}
%~\cite{cheng2022xmem,oh2019video,cheng2021rethinking,hu2021learning,lu2020video,mao2021joint,seong2020kernelized,seong2021hierarchical,xie2021efficient,ying2023ctvis}
% ~\cite{cai2022memot,hao2022umotma,xin2022multi,fang2018recurrent,allen2006multiple}
% ~\cite{zhou2023memory,fu2021stmtrack,yang2018learning,liu2017mavot,ma2018adaptive}

\vspace{-5pt}

\subsection{Memory Models in Vision Tasks}

\vspace{-3pt}

There are some prior works exploring memory models~\cite{squire2015memory} in various vision tasks in videos, such as video object segmentation~(VOS)~\cite{cheng2022xmem,hu2021learning,seong2020kernelized,seong2021hierarchical}, multi-object tracking~(MOT)~\cite{cai2022memot,hao2022umotma,xin2022multi,allen2006multiple}, visual object tracking~(VOT)~\cite{zhou2023memory,yang2018learning,liu2017mavot,ma2018adaptive}, and action understanding~\cite{wang2023memory}.
MeMOT~\cite{cai2022memot} builds a large spatiotemporal memory that stores the past observations of the
tracked objects. 
XMem~\cite{cheng2022xmem} develops an architecture that incorporates multiple independent yet deeply-connected feature memory storage to handle long videos with thousands of frames.
We learn from the experience of those prior arts and further adopt an effective memory mechanism in combination with LLMs. 
% Unlike using embedded feature given by certain visual encoders, we find that using tokens in Transformers~\cite{vaswani2017attention} as the carriers of memory suitable for both LLMs and ViT~\cite{dosovitskiy2020image} based visual encoder.
Our method focuses on reducing the redundancy of visual tokens in the video and building a memory mechanism to pass the information among a large temporal range.

==> tex/3_method.tex <==
\section{MovieChat}

\subsection{Overview}
Our proposed method, MovieChat, comprises several key components, including the frame-wise visual feature extractor, the short-term and long-term memory modules, the video projection layer, and the Large Language Model (LLM), as illustrated in Fig.~\ref{fig:overview}. MovieChat is designed for ultra-long videos ($\textgreater 10$K frames) understanding through interactive dialogue with the user. To address the impractical storage demands of concurrently storing a vast number of frames in both GPU memory and RAM, we employ a sliding window approach to efficiently process the video. The short-term memory module embeds dense tokens with sliding window and the long-term memory module periodically updates. MovieChat supports two inference modes: Breakpoint mode is used to understand a specific moment in the video, providing insights and answers based on that particular frame or scene; Global mode, on the other hand, is employed to comprehend the entire video as a whole, enabling a comprehensive understanding of the overall content and context.

\vspace{15pt}

\subsection{Visual Feature Extraction}
For visual feature extraction, instead of utilizing video-based foundational models such as ViViT~\cite{arnab2021vivit} or Video-Swin~\cite{liu2022video}, we simply use an image-based model to get frame-wise feature in the form of tokens. To be specific, we utilize pre-trained models as our visual feature extractor, including the ViT-G/14 from EVA-CLIP~\cite{fang2022eva} and the Q-former from BLIP-2~\cite{li2023blip2}. This is mainly because 1) there is few video foundation model that makes good alignment with text, and 2) our proposed memory mechanism can effectively capture temporal features. Given a raw video, the visual input $\mathbf{v} \in \mathbb{Z}^{T \times 3 \times H \times W}$ is a sequence of $T$ RGB frames of size $H \times W$ sampled from the video. The visual features are extracted in a sliding window manner, which could be formulated as
\begin{equation}
    B_{n} = \{ \mathbf{x}_{i}= \mathcal{V}(\mathbf{v}_{i}) \mid \forall i = 1,...,C\}, n = 1,...,\lceil \frac{T}{C} \rceil,
\end{equation}
where $B_{n}$ is the $n$-th video clip feature within the sliding window spanning $C$ frames. $\mathcal{V}(\cdot)$ is the visual feature extractor, taking as input a single frame {$\mathbf{v}_{i}\in \mathbb{Z}^{3 \times H \times W}$}. {$\mathbf{x}_{i}$} $\in \mathbb{R}^{N \times D}$ denotes $N$ extracted visual tokens with respect to each frame, and $D$ is the feature dimension of each token.

\vspace{2.5pt}

\subsection{Short-term Memory}
Short-term memory stores the frame tokens in a temporary fixed-length buffer. The previously extracted visual features by sliding window $G$ times without further processing are used to construct short-term memory, which can be formulated by:
\begin{equation}
    \mathcal{S} = \bigcup_{n}{B}_{n} = \{ \mathbf{{x}}_{i} \mid \forall i = 1, ..., K\}, n=1,..,G,
\end{equation}
where $\mathcal{S}$ is short-term memory, and $K$ is equal to $ C \times G$. Note that we set short-term memory to contain a fixed length of $K$ frames since the role of short-term memory is to assist in video understanding based on previous short-term contextual information. 

The update strategy for short-term memory is based on the First-in-First-out~(FIFO) queue. As a new batch of visual tokens enters, when the short-term memory reaches its capacity, we pop the currently stored frames to the memory consolidation module and clear the short-term memory. The output video feature obtained from the consolidation module augments the long-term memory; on the other hand, it reinitializes the short-term memory with this feature. The initialization aims at communicating the information between different sliding windows, thereby achieving more efficient compression.

\vspace{2.5pt}

\subsection{Long-term Memory}

Long-term memory can effectively avoid the problem of catastrophic knowledge forgetting, which is crucial for handling long video understanding tasks. The features stored in short-term memory are dense tokens, but due to the limitations of GPU memory and computation cost, storing all the tokens dropped from short-term memory into long-term memory buffer in sequence is infeasible. Besides, we observe significant temporal redundancy in videos, where activities span multiple frames with minimal visual changes. To this end, we propose a method to merge adjacent similar frames to simplify video feature representation and accelerate video encoding. This method transforms the dense tokens to the sparse memories, which are stored in long-term memory. 

\input{alg/longterm}

To be specific, as shown in Algorithm~\ref{alg:longterm}, we conduct memory consolidation by merging the most similar tokens in the adjacent frames following ToMe~\cite{bolya2022token} periodically. We find that the token embedding in Transformer already summarize the information of each frame for using in calculating the average cosine similarity $s$ of $N$ embedded tokens:
\begin{equation}
    s = \frac{1}{N} \sum_{j=1}^{N} \left [ \cos(\mathbf{x}_{i}^{j}, \mathbf{x}_{i+1}^{j}) \right ].
\end{equation}

Our goal is to keep $R_{L}$ frames after every merge operation, which also embeds rich information stored in the long-term memory. $R_{L}$ is the hyper-parameter to control the trade-offs between performance and efficiency. Therefore, we greedily merge each set of adjacent frames with the highest similarity via weighted averaging. The merge operation is iteratively conducted until the token count reaches the predefined value set $R_{L}$ for each consolidation operation, resulting in the output video feature $\mathbf{v'} \in \mathbb{Z}^{R_{L}\times 3 \times H \times W}$ (operational details in appendix). The above algorithm is parameter-free, and can be easily plugged into a frame-based video encoder. Although the frame similarity calculation brings additional computing overhead, it is negligible compared to the efficiency gained by reducing stored frames.


\paragraph{Extend positional encoding.} For long-term memory, the number of tokens exceeds the maximum length of the positional encoding from the pre-trained model. Thus, our model utilizes the positional encoding mechanism following BERT~\cite{kenton2019bert}, which results in a portion exceeding the length threshold $n$ without available positional encoding. In order to handle long enough long memory, we adopt the hierarchically decomposed positional encoding method proposed by Su~\etal~\cite{pos}, which allows to extend the absolute positional encoding of length from $n$ to $n^2$.

\subsection{Inference}

Previous methods always use the representation of the whole video to conduct understanding and question-answering, which may fail in localizing specific moment especially in long videos. To this end, we propose two inference modes, global and breakpoint, for long video understanding task as follows.

\input{fig/benchmark}
\input{fig/wordcloud}

\paragraph{Global mode.}

Global mode is defined as the understanding and question-answering for the whole video. In this case, we only use long-term memory $\mathcal{L}$ as the video representation $\mathbf{V}$.



\paragraph{Breakpoint mode.}

Breakpoint mode is distinctly defined as understanding specific moments in a video. Since events inherently possess continuity, we need to consider not only the information directly related to the moments stored in short-term memory $\mathcal{S}$ but also the information indirectly related stored in long-term memory $\mathcal{L}$. Based on this, we hypothesize that when querying the movie at a specific moment $t$, the video representation $\mathbf{V}$ should be the aggregation of $\mathcal{L}$, $\mathcal{S}$, and the current video frame feature $\mathbf{x}_{t}$. We find that simply concatenating these items yields excellent performance and leave further exploration of additional aggregation choices for future work.

\vspace{10pt}

Subsequently, the video representation $\mathbf{V}$ goes through a Q-former and a linear projection layer before being fed into the LLM $\mathcal{O}$, which can be formulated as:
\begin{equation}
    \mathbf{A} = \mathcal{O}(\mathbf{Q}, \mathcal{P} (\mathbf{V})),
\end{equation}
where $\mathcal{P}$ is the projection from visual space to text space. $\mathbf{A}$ represents the answer or instruction, and $\mathbf{Q}$ is employed to denote the question, respectively.

\vspace{15pt}

==> tex/4_dataset.tex <==
\vspace{5pt}
\section{A New Benchmark: MovieChat-1K}

\vspace{-5pt}

Previous works on building long video understanding benchmarks either focus on non-question-answering tasks~(\eg, language grounding~\cite{soldan2022mad}, generic event boundary detection~\cite{shou2021generic}, user engagement and movie metadata prediction~\cite{wu2021towards}, \etc) or lack long-form understanding evaluation~\cite{huang2020movienet}. To better evaluate the performance of MovieChat, we collect a new benchmark for long video understanding tasks, MovieChat-1K, which contains 1K high quality video clips sourced from various movies and TV series with 14K manual annotations. 

As shown in Fig.~\ref{fig:category}, we collect videos from 15 popular categories with varying distribution, including documentary film, detective film, animation film, and so on. Among these, each video comprises multiple alternating scenes, contributing to a diverse and dynamic visual narrative within the context of the collection. The visual representation in Fig.~\ref{fig:video_length} demonstrates the clip duration distribution of MovieChat-1K. Over 90\% of the videos exhibit a duration ranging from 10K to 12K frames, while 14.6\% of videos extending beyond 12K frames. Only 8.6\% of videos have duration less than 10k frames.



% Fig.~\ref{fig:category} and Fig.~\ref{fig:length} demonstrate the category and the clip length statistics compared to other benchmarks. 

For each video, we manually set and provide 1 dense caption for the whole video, 3 question-answering pairs for global mode and 10 question-answering pairs with timestamps for breakpoint mode. Fig.~\ref{fig:question_type} illustrates the distribution of question types in MovieChat-1K. Note that MovieChat-1K is specifically designed for long video comprehension tasks, the majority of questions are open-ended, with only a quarter classified as multiple-choice questions, marked by initiators such as `Do,' `Does,' `Is,' or `Are.' We also compute the word distributions of our provided question-answer pairs. As illustrated in  Fig.~\ref{fig:wordcloud}, which includes common objects (people, clothes, etc.), time (day, night, etc.), scenes (indoor, outdoor, etc.), and so on.
More statistics information can be found in appendix.


\vspace{-5pt}



==> tex/5_exp.tex <==
\vspace{8pt}
\input{tab/short}
\input{tab/short_varies}
\section{Experiments}

\vspace{-5pt}

We conduct quantitative and qualitative evaluations between MovieChat and previous methods. Additionally, we perform ablation studies to investigate MovieChat. Experimental settings and analyses can be found in appendix.

\subsection{Quantitative Evaluation}



\label{exp:quantitative}


\paragraph{Short video question-answering.} We use several widely used open-ended datasets: MSVD-QA~\cite{xu2017video}, MSRVTT-QA~\cite{xu2016msr-vtt}, and ActivityNet-QA~\cite{yu2019activitynet} for short video question-answering tasks. The evaluation process is under the assistance of LLM with the default hyper-parameter settings. The accuracy and relative scores on a scale of $0$ to $5$ are reported. Compared to previous methods~\cite{maaz2023video,li2023videochat,zhang2023llama, zhang2023video}, MovieChat achieves comparable performance even it is not specifically designed for short video question-answering tasks, as shown in Tab.~\ref{tab:short}.



\vspace{-12pt}

\paragraph{Short video generative performance.} Following ~\cite{maaz2023video}, we employ GPT-assisted evaluation to conduct a more comprehensive comparison of the text generation performance between MovieChat and previous methods~\cite{maaz2023video,li2023videochat,yang2022zero} on processed ActivityNet-QA~\cite{yu2019activitynet}. The evaluation pipeline covers crucial metrics (including \textit{Correctness of Information}, \textit{Detailed Orientation}, \textit{Contextual Understanding}, \textit{Temporal Understanding} and \textit{Consistency}) and assigns relative scores to the generated predictions on a scale of 1-5. We present the results of the generation performance evaluation in Tab.~\ref{tab:short_varies}. The results reveal its competitive performance across all key aspects compared to previous methods. 






\vspace{-12pt}

\paragraph{Long video question-answering.} We evaluate the long video question-answering performance of MovieChat with our proposed MovieChat-1K. We split 1,000 videos into training set~(800), test set~(100), validation set~(100) and only use test set for final performance evaluation. We select three recent LLM-based video understanding models~(\eg Video Chat~\cite{li2023videochat}, Video LLaMA~\cite{zhang2023video}, and Video-ChatGPT~\cite{maaz2023video}) as the baselines. Yet, none of those methods can support such long video~($\textgreater 10$K frames). Therefore, to accommodate their length limitations in global questions, we uniformly sample from the original video up to the maximum frame count which can be officially supported by each individual model. For breakpoint questions, we extend half of the maximum frame count before and after the breakpoint (\ie, placing the breakpoint at the center frame). 

\input{tab/long}
\input{tab/long_varies}
\input{fig/ablation}
To enhance the robustness of the results, we simultaneously employ GPT-3.5~\cite{gpt3.5} and Claude~\cite{examplewebpage} as LLM assistants, with the additional support of human blind rating. We observe a discrepancy between the accuracy and relative score generated by the previously LLM-assisted evaluation method~\cite{maaz2023video} for video question-answering tasks. However, merely adjusting the prompt for the LLM cannot effectively address this issue. Therefore, after obtaining the accuracy and score from the LLM-assisted evaluation method, we implement manual filtering to remove results with inconsistent values, thus improving the reliability of our outcomes.


As shown in Tab.~\ref{tab:long}, compared to previous methods~\cite{maaz2023video,li2023videochat,zhang2023video}, MovieChat reads more video frames. In both global mode and breakpoint mode, our method maintains a performance gain in terms of the average accuracy and score provided by LLM assistants and human blind rating. We comprehensively evaluate MovieChat's question-answering performance across different question types compared to baselines. The results indicate that our approach outperforms the baselines in both open-ended and true-false questions.



\vspace{-8pt}

\paragraph{Long video generative performance.} 

We compare the quality of answers generated by MovieChat and previous methods~\cite{maaz2023video,li2023videochat,zhang2023video} in long video question-answering on MovieChat-1K. As shown in Tab.~\ref{tab:long_varies}, with the average score provided by GPT-3.5~\cite{gpt3.5}, Claude~\cite{examplewebpage} and human bling rating, our approach continues to generate higher-quality answers even as the video contents become more extensive.


\subsection{Ablation Study}



\input{tab/videollama_score}

\vspace{-8pt}

\paragraph{Short-term and long-term memory buffers.} 
As MovieChat incorporates a memory mechanism including short-term memory and long-term memory, it is imperative to evaluate how the proposed memory mechanism influences the performance. Tab.~\ref{tab:videollama_score} and Tab.~\ref{tab:videollama_5} provide the memory-dependent performance of MovieChat for long video question-answering and generative tasks with the average results of GPT-3.5~\cite{gpt3.5}, Claude~\cite{examplewebpage}, and human blind rating. MovieChat with the memory mechanism significantly outperforms the memory-independent variant, which signifies the importance of memory mechanisms.

\vspace{-8pt}

\paragraph{Hyper-parameter ablations.} 
We perform a series of hyperparameter ablations based on the MovieChat-1K dataset to better understand MovieChat. Fig.~\ref{fig:ablation} shows the performance when ablating the length of memory buffers, consolidation length and short-term initialization with the average results of GPT-3.5~\cite{gpt3.5}, Claude~\cite{examplewebpage}, and human blind rating. The performance of MovieChat degrades when all four are significantly changed, showing the validity of our empirically chosen hyperparameyers. Fig.~\ref{fig:ablation} demonstrates that information obtained from the video expands with the growing length of memory buffers, while the loss of finer details intensifies with the fixed length of consolidation. Furthermore, using merged tokens for short-term initialization outperforms last few tokens and uniform sampling. Additionally, the length of merged tokens and the memory buffer size have a combined effect on MovieChat's performance.

\definecolor{global}{RGB}{21,96,130}
\definecolor{breakpoint}{RGB}{51,0,111}

\input{tab/videollama_5}

\vspace{-8pt}

\subsection{Case Study}

\vspace{-7pt}

We perform an extensive case study of MovieChat on a variety of open-ended long video~(such as cartoon movie and TV series) for long video question-answering, including the \parbox[c][8pt][l]{8pt}{\colorbox{breakpoint}{}}breakpoint mode (Q\#1) and the \parbox[c][8pt][l]{8pt}{\colorbox{global}{}}global mode (Q\#2). The evaluation is conducted between MovieChat and previous methods~\cite{maaz2023video,li2023videochat,zhang2023llama} as shown in Fig.~\ref{fig:case} . For Q\#1 in breakpoint mode, we mark the timestamp when the question is asked. For long videos over $10$K frames, MovieChat is still capable of providing excellent responses to questions regarding both the current moment and the entire video content with less hallucination. More examples to show long video scene understanding and temporal understanding ability of MovieChat are available in appendix. 

\input{fig/case}


==> tex/6_conclusion.tex <==
\section{Limitation}

Although MovieChat has demonstrated impressive abilities in long video understanding, it is still an early-stage prototype and has some limitations, including: 1) Limited perception capacities. MovieChat’s performance is hindered by the pretrained short video understanding model. 2) Inadequate Time Processing. MovieChat provides only rough estimates of the duration proportions of events within long videos, lacking precision in temporal details.

\section{Conclusion}

Conclusively, we presents an innovative video understanding system integrating video foundation models and large language models. By incorporating a memory mechanism represented by tokens in Transformers, our proposed system, MovieChat overcomes challenges associated with analyzing long videos.
MovieChat achieves state-of-the-art performance in long video understanding, surpassing existing systems limited to handling videos with few frames. 

% The study emphasizes the significance of memory mechanisms in video understanding, enabling the model to retain and retrieve relevant information over extended duration. MovieChat's success has practical implications in domains like video surveillance, content analysis, and video recommendation systems.
% Future research can explore further improvements to the memory mechanism and the integration of other modalities, such as audio, to enhance video understanding capabilities. This work opens up opportunities for applications requiring a comprehensive understanding of long-term visual information.
